Improving Backward Conformal Prediction via Non-Conformity Score Transformation

Conformal Prediction (CP) provides a statistical framework for uncertainty quantification that constructs prediction sets with coverage guarantees. While CP yields uncontrolled prediction set sizes, Backward Conformal Prediction (BCP) inverts this paradigm by enforcing a predefined upper bound on set size and estimating the resulting coverage guarantee. However, the looseness induced by Markov's inequality within the BCP framework causes a significant gap between the estimated coverage bound and the empirical coverage. In this work, we introduce ST-BCP, a novel method that introduces a data-dependent transformation of nonconformity scores to narrow the coverage gap. In particular, we develop a computable transformation and prove that it outperforms the baseline identity transformation. Extensive experiments demonstrate the effectiveness of our method, reducing the average coverage gap from 4.20\% to 1.12\% on common benchmarks.

==> section/limitations.tex <==
\section{Limitations}
 The theoretical assumptions underlying this method remain notably complex, particularly in cases where size constraint rules depend simultaneously on features and the calibration set.  Additionally, while the derivation of the optimal transformation ensures the consistency of the estimator, it did not consider estimation efficiency.
